Automated Localization of Blood Vessels in Retinal Images

Vessel structure is one of the most important parts of the retina which physicians can detect many diseases by analysing its features. Localization of blood vessels in retina images is an important process in medical image analysis. This process is also more challenging with the presence of bright and dark lesions. In this thesis, two automated vessel localization methods to handle both healthy and unhealthy (pathological) retina images are analyzed. Each method consists of two major steps and the second step is the same in the two methods. In the first step, an algorithm is used to decrease the effect of bright lesions. In Method 1, this algorithm is based on K- Means segmentation, and in Method 2, it is based on a regularization procedure. In the second step of both methods, a multi-scale line operator is used to localize the line-shaped vascular structures and ignore the dark lesions which are generally assumed to have irregular patterns. After the introduction of the methods, a detailed quantitative and qualitative comparison of the methods with one another as well as the state-of-the-art solutions in the literature based on the segmentation results on the images of the two publicly available datasets, DRIVE and STARE, is reported. The results demonstrate that the methods are highly comparable with other solutions.

==> app.tex <==
\appendix

%%%%%%%%%% DON'T DELETE THIS, REVERTS NUMBERING BACK %%%%%%%%%%%%%
\makeatletter
\renewcommand{\@makechapterhead}[1]{\vspace *{-10\p@ }{\parindent \z@ 
\raggedright \normalfont \ifnum \c@secnumdepth >\m@ne \Huge \bfseries 
\@chapapp \space \thechapter \vskip 10\p@ \fi #1\par \nobreak \vskip 30\p@ }}
\makeatother
%%%%%%%%%% DON'T DELETE THIS, REVERTS NUMBERING BACK %%%%%%%%%%%%%

\chapter{}
\vspace*{-0.3in}
\begin{figure}[hb!]
\begin{center}
\makebox[\textwidth][c]{\includegraphics[width=1.0\textwidth]{costperMb2015_4.jpg}}
\end{center}
\caption[Cost per raw megabase of DNA sequence from 2001 to 2015]{Cost per raw megabase of DNA sequence from 2001 to 2015. Straight line - Moore's Law, blue curve - cost in US dollars, Y-axis scale is logarithmic. Graph reproduced from \citep{wetterstrand2016}}
\end{figure}
\begin{figure}[hb!]
\begin{center}
\makebox[\textwidth][c]{\includegraphics[width=1.0\textwidth]{costperMb2015_4.jpg}}
\end{center}
\caption[Cost per raw megabase of DNA sequence from 2001 to 2015]{Cost per raw megabase of DNA sequence from 2001 to 2015. Straight line - Moore's Law, blue curve - cost in US dollars, Y-axis scale is logarithmic. Graph reproduced from \citep{wetterstrand2016}}
\end{figure}

\chapter{}
\vspace*{-0.3in}
\begin{figure}[hb!]
\begin{center}
\makebox[\textwidth][c]{\includegraphics[width=1.0\textwidth]{costperMb2015_4.jpg}}
\end{center}
\caption[Cost per raw megabase of DNA sequence from 2001 to 2015]{Cost per raw megabase of DNA sequence from 2001 to 2015. Straight line - Moore's Law, blue curve - cost in US dollars, Y-axis scale is logarithmic. Graph reproduced from \citep{wetterstrand2016}}
\end{figure}

\chapter{}
\begin{figure}[hb!]
\begin{center}
\includegraphics[scale=0.5]{costperMb2015_4.jpg}
\end{center}
\caption[Cost per raw megabase of DNA sequence from 2001 to 2015]{Cost per raw megabase of DNA sequence from 2001 to 2015. Straight line - Moore's Law, blue curve - cost in US dollars, Y-axis scale is logarithmic. Graph reproduced from \citep{wetterstrand2016}}
\end{figure}

\chapter{}
\begin{figure}[hb!]
\begin{center}
\includegraphics[scale=0.5]{costperMb2015_4.jpg}
\end{center}
\caption[Cost per raw megabase of DNA sequence from 2001 to 2015]{Cost per raw megabase of DNA sequence from 2001 to 2015. Straight line - Moore's Law, blue curve - cost in US dollars, Y-axis scale is logarithmic. Graph reproduced from \citep{wetterstrand2016}}
\end{figure}

\chapter{}
\begin{figure}[hb!]
\begin{center}
\includegraphics[scale=0.5]{costperMb2015_4.jpg}
\end{center}
\caption[Cost per raw megabase of DNA sequence from 2001 to 2015]{Cost per raw megabase of DNA sequence from 2001 to 2015. Straight line - Moore's Law, blue curve - cost in US dollars, Y-axis scale is logarithmic. Graph reproduced from \citep{wetterstrand2016}}
\end{figure}


